Polytypic Quantum Wells in Si and Ge: Impact of 2D Hexagonal Inclusions on Electronic Band Structure

Crystal defects, traditionally viewed as detrimental, are now being explored for quantum technology applications. This study focuses on stacking faults in silicon and germanium, forming hexagonal inclusions within the cubic crystal and creating quantum wells that modify electronic properties. By modeling defective structures with varying hexagonal layer counts, we calculated formation energies and electronic band structures. Our results show that hexagonal inclusions in Si and Ge exhibit a direct band gap, changing with inclusion thickness, effectively functioning as quantum wells. We find that Ge inclusions have a direct band gap and form Type-I quantum wells. This research highlights the potential of manipulating extended defects to engineer the optoelectronic properties of Si and Ge, offering new pathways for advanced electronic and photonic device applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
